A Likelihood Ratio-Based Approach to Segmenting Unknown Objects

Addressing the Out-of-Distribution (OoD) segmentation task is a prerequisite for perception systems operating in an open-world environment. Large foundational models are frequently used in downstream tasks, however, their potential for OoD remains mostly unexplored. We seek to leverage a large foundational model to achieve robust representation. Outlier supervision is a widely used strategy for improving OoD detection of the existing segmentation networks. However, current approaches for outlier supervision involve retraining parts of the original network, which is typically disruptive to the model's learned feature representation. Furthermore, retraining becomes infeasible in the case of large foundational models. Our goal is to retrain for outlier segmentation without compromising the strong representation space of the foundational model. To this end, we propose an adaptive, lightweight unknown estimation module (UEM) for outlier supervision that significantly enhances the OoD segmentation performance without affecting the learned feature representation of the original network. UEM learns a distribution for outliers and a generic distribution for known classes. Using the learned distributions, we propose a likelihood-ratio-based outlier scoring function that fuses the confidence of UEM with that of the pixel-wise segmentation inlier network to detect unknown objects. We also propose an objective to optimize this score directly. Our approach achieves a new state-of-the-art across multiple datasets, outperforming the previous best method by 5.74% average precision points while having a lower false-positive rate. Importantly, strong inlier performance remains unaffected.

==> tables/SMIYC.tex <==
\begin{table*}[t!]
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{l c c c c c c c c c c } 
    \toprule
    \multirow{2}{*}{Method}  & \multicolumn{5}{c}{Anomaly Track}  & \multicolumn{5}{c}{Obstacle Track} \\      \cmidrule(lr){2-6} \cmidrule(l){7-11}
           & $AP$ $\uparrow$ & $FPR$ $\downarrow$ & $sIoU_{gt}$ $\uparrow$ & $PPV$ $\uparrow$ & $\overline{F_1}$ $\uparrow$ & $AP$ $\uparrow$  & $FPR$ $\downarrow$ & $sIoU_{gt}$ $\uparrow$ & $PPV$ $\uparrow$ &  $\overline{F_1}$ $\uparrow$ \\
    \midrule

     cDNP~\cite{Galesso2023ICCVW} & 88.90 & 11.42 & 50.44 & 29.04  & 28.12 & - & -  & - & - & - \\
     Maskomaly~\cite{Ackermann2023BMVC}  & 93.35 & 6.87 & 55.43 & 51.46  & 49.90 & - & -  & - & - & - \\ % I guess this can also be removed from this table as they only evaluate on Anomaly Track
     Mask2Anomaly~\cite{Rai2023ICCV} & 88.72 & 14.63 & 55.28 & 51.68  & 47.16 & 93.22 & 0.20  & 55.72 & 75.42 & 68.15 \\
     
     EAM~\cite{Grcic23CVPRW}  & 93.75 & 4.09 & 67.09 & 53.77  & 60.86 & 92.87 &0.52  & 65.86 & 76.50 & 75.58 \\
     RbA~\cite{Nayal2023ICCV} & 94.46 & 4.60 & 64.93 & 47.51  & 51.87 & 95.12 & 0.08 & 54.34 & 59.08 & 57.44 \\ 
     \midrule
     Ours & 95.6 & 4.7 & 57.9 & 41.2  & 43.3 & 	94.4 & 0.1 & 49.8 & 76.8 & 67.2\\
     \bottomrule
    \end{tabular}}
    \caption{\textbf{Results on the SMIYC benchmark.} } %
    
    \label{tab:smiyc}
\end{table*}

==> tables/backbone_ablation.tex <==
%\begin{wraptable}{r}{0.5\textwidth}
%    \centering
%    \adjustbox{max width=0.5\textwidth}{
%    \begin{tabular}{c|c||ccc}
%        \hline
%        & \textbf{Cityscapes} & \multicolumn{3}{c}{\textbf{RoadAnomaly}} \\
%        \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Backbone}}} & {mIoU}$\uparrow$ & AUROC$\uparrow$ & AP$\uparrow$ & FPR$_{95}\!\downarrow$ \\ \hline\hline
%        dinoV2-b & - & - & - & - \\
%        Segformer & - & - & - & - \\
%        \hline
%    \end{tabular}}
%    \caption{Caption for the table.}
%    \label{tab:backbone_ablation}
%\end{wraptable}

\begin{table}[h]
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{l c c c c c c c } 
     \toprule
     \multirow{2}{*}{Backbone} &\multicolumn{1}{c}{Cityscapes}  & \multicolumn{3}{c}{Road Anomaly} & \multicolumn{3}{c}{FS LaF}  \\
        \cmidrule(r){3-5} \cmidrule(l){6-8}
        & $mIoU$ $\uparrow$ & $AUROC$ $\uparrow$ & $AP$ $\uparrow$ & $FPR$ $\downarrow$ & $AUROC$ $\uparrow$ & $AP$ $\uparrow$ & $FPR$ $\downarrow$ \\
         \midrule
        Deeplab$_{V3}$& 81.1  & 84.71 & 34.42	& 47.90  & 97.34 & 43.47 & 13.11 \\  
        FCN & 76.7  & 78.99 &  24.51 & 56.95 & 96.28 & 32.94 &  16.07 \\
        Segformer~\cite{xie2021NeurIPS} & 82.6  & 89.37 & 57.65 &  44.34 & 97.83 &  50.03 & 12.55 \\
        Swin-b & 81.6  & 79.93 & 35.77 &  66.53 & 83.00 &  5.83 & 68.83 \\
        % \midrule
        DinoV2-b~\cite{Oquab2024TMLR} & 81.\todo{?} & 92.94 &64.77  & 28.25 & 90.83 & 15.00 & 40.70\\
         \bottomrule   
        \end{tabular}}
        \caption{\textbf{GMMSeg with Different Backbones.} 
        } \todo{What was the cityscapes performance for the best model?}
        \label{tab:backbone_ablation}
\end{table}

==> tables/component_level_metrics.tex <==
\begin{table*}[h]
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{l l c c c c c c|| c c c} 
    \toprule
      \multicolumn{2}{c}{CLS Head} & \multicolumn{3}{c}{SMIYC-AT}  & \multicolumn{3}{c}{SMIYC-OT} & \multicolumn{3}{c}{Average} \\
    \cmidrule(lr){3-5} \cmidrule(l){6-8}  \cmidrule(l){9-11}
          \multicolumn{2}{c}{X-Y}  & $sIoU_{gt}$ $\uparrow$ & $PPV$ $\uparrow$ & $\overline{F_1}$ $\uparrow$  & $sIoU_{gt}$ $\uparrow$ & $PPV$ $\uparrow$ & $\overline{F_1}$ $\uparrow$ & $sIoU_{gt}$ $\uparrow$ & $PPV$ $\uparrow$ & $\overline{F_1}$ $\uparrow$  \\
    \midrule
    \multicolumn{2}{c}{G-G} & 56.7 & 51.5 & 50.7 & 42.6 & 59.2 & 50.9 & 49.7 & 55.4 &50.8\\
    \multicolumn{2}{c}{G-D}  & 52.0 & 39.9 & 36.6 & 41.4 & 70.7 & 56.9 & 46.7 & 55.3&46.8\\
     \multicolumn{2}{c}{D-D} & 57.9 & 41.2 & 43.3 & 	49.8 & 76.8 & 67.2 & 53.9 & 59.0 &55.3\\
     %\hline
     %\multicolumn{11}{c}{Other approaches}\\
     %\hline
     %\multicolumn{2}{c}{RbA} & 55.7 & 52.1 & 46.8 & 58.4& 58.8& 60.9 & 57.1 & 55.5&53.9\\
     \bottomrule
    \end{tabular}}
    \vspace{5pt}
    \caption{\textbf{Component-Level Metrics.} We report the component-level metrics on the SMIYC-AT and SMIYC-OT for both the discriminative~(D) and generative~(G) models for the classification head (X) and unknown estimation module (Y).}
    \label{tab:component}
\end{table*}

==> tables/genv_vs_discr.tex <==
\begin{table*}[h]
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{l l c c c c c c c c|| c c } 
    \toprule
      \multicolumn{2}{c}{CLS Head} & \multicolumn{2}{c}{SMIYC-AT}  & \multicolumn{2}{c}{SMIYC-OT} & \multicolumn{2}{c}{ Road Anomaly}  & \multicolumn{2}{c||}{FS LaF} & \multicolumn{2}{c}{Average} \\
    \cmidrule(lr){3-4} \cmidrule(l){5-6} \cmidrule(lr){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12}
          \multicolumn{2}{c}{X-Y}  & $AP$ $\uparrow$ & $FPR$ $\downarrow$ & $AP$ $\uparrow$  & $FPR$ $\downarrow$ & $AP$ $\uparrow$ & $FPR$ $\downarrow$ & $AP$ $\uparrow$  & $FPR$ $\downarrow$ & $\overline{AP}$ $\uparrow$  & $\overline{FPR}$ $\downarrow$  \\
    \midrule
    \multicolumn{2}{c}{UEM (G-G)} & 94.1 & 6.9 & 88.3 & 0.40 & 93.75 & 6.32 & 71.34 & 6.04 & 86.87 & 4.92 \\
    \multicolumn{2}{c}{UEM (G-D)}  & 92.50 & 11.3 & 92.0 & 0.20 & 92.86 & 8.95 & 79.02 & 1.62 & 89.10 & 5.52\\
     \multicolumn{2}{c}{UEM (D-D)} & 95.6 & 4.70 & 94.40 & 0.10 & 90.94 & 8.03 & 72.83 & 2.60 & 88.44 & 3.86 \\
     \bottomrule
    \end{tabular}}
    \caption{\textbf{Discriminative vs. Generative Modeling.} In our model, we have the flexibility to use a discriminative~(D) or generative~(G) modeling for the inlier classification head (X) and unknown estimation module (Y). We report the results of three possible combinations.}
    \label{tab:gen_vs_dis}
\end{table*}

==> tables/implementation_details.tex <==
\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c}
        \hline
        \multicolumn{2}{c|}{\textbf{Hyperparameter}}  & \textbf{Value}\\
        \hline
        \multicolumn{2}{c|}{batch\_size}&16\\
         %\multicolumn{2}{c}{precision}&bf16-mixed\\
         \multicolumn{2}{c|}{max\_steps}&40000\\
         \multicolumn{2}{c|}{eval\_window\_size}&[518,1036]\\
         \multicolumn{2}{c|}{eval\_stride}&[140,140]\\
         \hline
        
         \multirow{2}{*}{Backbone} &model & DinoV2~\cite{Oquab2024TMLR}\\
         & version &  VitB14Reg~\cite{Darcet2024ICLR}\\
        \hline
        \multirow{4}{*}{Pixel Decoder} &model & FPN~\cite{Lin2017CVPR}\\
         & depth & 4\\
         & feature\_indicies & [1,4,8,11] \\
         &output\_dimension& 256\\
         \hline
         \multirow{7}{*}{GMM Head} & num\_components\_per\_class & 5 \\
         & update\_interval & 5 \\
         & gamma\_mean & 0.999 \\
         & gamma\_conv & 0 \\
         & memory\_size & 8000 \\
         &sinkhorn\_factors & [1,1,1] \\
         &max\_sample\_size & 20 \\
         \hline
         \multirow{1}{*}{Linear Head}&hidden\_size & 256 \\
         \hline
         \multirow{3}{*}{Optimizer} & type & AdamW~\cite{Loshchilov2019ICLR} \\
         &learning\_rate &$5e-4$ \\
         &weight\_decay &0.0 \\
         \hline
         \multirow{3}{*}{LR Schedule} & type & PolyWithLinearWarmup \\
         & num\_warmup\_steps&1500\\
         &lr\_end&$1e-7$\\
         \hline
         \multirow{3}{*}{Fine-Tunning} & max\_steps & 4000 \\
         & proxy\_size&30000\\
         &ood\_prob&1.0\\
         
         
    \end{tabular}
    }
    \vspace{5pt}
    \caption{\textbf{A Summary of Hyper-parameters Used for Experiments.}}
    \label{tab:implement_details}
\end{table}

==> tables/ra_fs_lr.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l c c c c } 
     \toprule
     % I removed AUC because most of the newer methods don't report it. 
     \multirow{2}{*}{Method} & \multicolumn{2}{c}{Road Anomaly} & \multicolumn{2}{c}{FS LaF}  \\
        \cmidrule(r){2-3} \cmidrule(l){4-5}
        & $AP$ $\uparrow$ & $FPR$ $\downarrow$ & $AP$ $\uparrow$ & $FPR$ $\downarrow$ \\
         \midrule
        cDNP~\cite{Galesso2023ICCVW}  & 79.78 & 18.18   & 69.80 &   7.50 \\
        UGainS~\cite{Nekrasov2023GCPR} & \underline{88.98} & 10.42  & \underline{80.08} & 6.61 \\
        %Maskomaly~\cite{Ackermann2023BMVC}  & - & 70.90 & 11.90  & - & - &  - \\ % I guess this will be removed from this table as they only evaluate on Road Anomaly?
        Mask2Anomaly~\cite{Rai2023ICCV}  & 79.70	& 13.45   & 46.04 &  4.36 \\  
        EAM~\cite{Grcic23CVPRW}  & 69.40	& \underline{7.70}  & \textbf{81.50} &  \underline{4.20} \\
        RbA~\cite{Nayal2023ICCV}  & 85.42 & \textbf{6.92} & 70.81 & 6.30 \\
        \midrule
        Ours  & \textbf{92.86} & 8.95 & 79.02 &\textbf{1.62}\\
         \bottomrule   
        \end{tabular}
        \caption{\textbf{Results on Road Anomaly and Fishyscapes LaF.} \dots The best and second best results are \textbf{bold} and \underline{underlined}, respectively.
        } % Currently, the best model found is inlier GMMseg linear OoD head path: augmented_linear_LOSS_1_LLR_3_comp5_warmup1500steps_gmmloss_0.0/step=1450-llr_AUPR=0.9331.ckpt
        \label{tab:ra_fs_lr}
\end{table}
